Strongly Polynomial Time Complexity of Policy Iteration for $L_\infty$ Robust MDPs

Markov decision processes (MDPs) are a fundamental model in sequential decision making. Robust MDPs (RMDPs) extend this framework by allowing uncertainty in transition probabilities and optimizing against the worst-case realization of that uncertainty. In particular, $(s, a)$-rectangular RMDPs with $L_\infty$ uncertainty sets form a fundamental and expressive model: they subsume classical MDPs and turn-based stochastic games. We consider this model with discounted payoffs. The existence of polynomial and strongly-polynomial time algorithms is a fundamental problem for these optimization models. For MDPs, linear programming yields polynomial-time algorithms for any arbitrary discount factor, and the seminal work of Ye established strongly--polynomial time for a fixed discount factor. The generalization of such results to RMDPs has remained an important open problem. In this work, we show that a robust policy iteration algorithm runs in strongly-polynomial time for $(s, a)$-rectangular $L_\infty$ RMDPs with a constant (fixed) discount factor, resolving an important algorithmic question.

==> homotopy_figure.tex <==
\begin{figure}[t]
    \centering
    \begin{tikzpicture}[scale=1.1, >=Stealth]

    % --- Setup ---
    % x-axis: Successor States sorted by Value v(s)
    % y-axis: Probability Mass p(s)

    % --- Axes ---
    % Extended x-axis to make room for the legend on the right
    \draw[->, thick] (-0.5,0) -- (9.0,0) node[right, font=\bfseries] {States (sorted by $v(s) \downarrow$)};
    \draw[->, thick] (0,-0.5) -- (0,3.5) node[above] {\textbf{Probability} $\mathbf{p_s}$};

    % --- Parameters ---
    \def\nomcolor{gray!20}
    \def\addcolor{blue!20}
    \def\subcolor{red!20}

    % --- Bar 1: s_hi (High Value, Full Increase) ---
    \node at (0.6, -0.3) {$s_{1}$};
    % Nominal
    \draw[fill=\nomcolor] (0.2,0) rectangle (1.0, 1.2);
    \node at (0.6, 0.6) {$\hat{P}$};
    % Increase
    \draw[fill=\addcolor, pattern=north east lines, pattern color=blue] (0.2,1.2) rectangle (1.0, 1.9);
    % Moved further left with xshift
    \node[blue, font=\tiny, left, xshift=-0.1cm] at (0.15, 1.55) {Mass Added};
    % Constraint Line
    \draw[red, dashed, thick] (0.1, 1.9) -- (1.1, 1.9);
    \node[red, above, font=\tiny] at (0.6, 1.9) {$\hat{P} + \delta$};

    % --- Bar 2: Intermediate (Full Increase) ---
    \node at (2.0, -0.3) {$s_2$};
    \draw[fill=\nomcolor] (1.6,0) rectangle (2.4, 0.8);
    \draw[fill=\addcolor, pattern=north east lines, pattern color=blue] (1.6,0.8) rectangle (2.4, 1.5);
    \draw[red, dashed, thick] (1.5, 1.5) -- (2.5, 1.5);

    % --- Bar 3: Pivot State (Partial Change) ---
    \node at (3.4, -0.3) {$s_{3}$};
    \draw[fill=\nomcolor] (3.0,0) rectangle (3.8, 1.0);

    % --- Bar 4: Intermediate (Full Decrease) ---
    \node at (4.8, -0.3) {$s_4$};
    % Remaining
    \draw[fill=\nomcolor] (4.4,0) rectangle (5.2, 0.4);
    % Removed
    \draw[dashed] (4.4,0.4) rectangle (5.2, 1.1);
    \draw[fill=\subcolor, pattern=north west lines, pattern color=red, opacity=0.5] (4.4,0.4) rectangle (5.2, 1.1);
    \draw[red, dashed, thick] (4.3, 0.4) -- (5.3, 0.4);
    \node[red, above, font=\tiny] at (4.8, 0.4) {$\hat{P} - \delta$};

    % --- Bar 5: s_lo (Low Value, Full Decrease) ---
    \node at (6.2, -0.3) {$s_{5}$};
    % Remaining (hit 0 or lower bound)
    \draw[fill=\nomcolor] (5.8,0) rectangle (6.6, 0.2);
    % Removed
    \draw[dashed] (5.8,0.2) rectangle (6.6, 0.9);
    \draw[fill=\subcolor, pattern=north west lines, pattern color=red, opacity=0.5] (5.8,0.2) rectangle (6.6, 0.9);
    \node[red, font=\tiny, right] at (6.6, 0.55) {Mass Removed};
    \draw[red, dashed, thick] (5.7, 0.2) -- (6.7, 0.2);

    % --- Arrows indicating flow ---
    % Control points lifted significantly higher (y=3.5) to clear all text/math
    \draw[->, ultra thick, blue, shorten >= 2pt, shorten <= 2pt] (6.2, 1.2) .. controls (6.2, 3.5) and (0.6, 3.5) .. (0.6, 2.1) node[midway, above, font=\small, black, yshift=0.1cm] {Transfer Mass from Low $v$ to High $v$};

    % --- Algorithm Description Box ---
    \node[align=left, font=\footnotesize, draw=black!50, rounded corners, fill=white, anchor=north west] at (7.0, 3.5) {
    \textbf{Homotopy Algorithm \ref{algo:homotopy}:}\\[0.3em]
    1. Sort states $s$ by value $v(s)$ desc.\\
    2. Initialize pointers $hi \leftarrow 1, lo \leftarrow |S|$.\\
    3. Shift mass from $s_{lo}$ to $s_{hi}$ within\\
    \hspace{1em} box $[\hat{P}-\delta, \hat{P}+\delta]$ and $\ge 0$.\\
    4. Move $hi/lo$ inward if limits hit.
    };

    \end{tikzpicture}
    \caption{Visualization of the Homotopy Algorithm \ref{algo:homotopy}.}
    \label{fig:homotopy}
\end{figure}
